Efficient Trace for RISC-V: Design, Evaluation, and Integration in CVA6

In this work, we present the design and evaluation of a Processor Tracing System compliant with the RISC-V Efficient Trace specification for Instruction Branch Tracing. We integrate our system into the host domain of a state-of-the-art edge architecture based on CVA6. The proposed Tracing System introduces a total overhead of 9.2% in terms of resource utilization on a Xilinx VCU118 FPGA on the CVA6 subsystem while achieving an average compression rate of 95.1% on platform-specific tests, compared to tracing each full opcode instruction.

==> figures/shaheen.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/img/shaheen_arch.pdf}
    \caption{Shaheen host-domain extended with TS.}
    \label{fig:shaheen}
    \vspace{-2mm}
\end{figure}

==> figures/te.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/img/TE_arch.pdf}
    \caption{Trace Encoder architecture.}
    \label{fig:te}
    \vspace{-2mm}
\end{figure}
